An Introduction to Permutation Processes (version 0.5)

These lecture notes were prepared for a special topics course in the Department of Statistics at the University of Washington, Seattle. They comprise the first eight chapters of a book currently in progress.

==> chapters/acknowledgements.tex <==
\extrachap{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}



==> chapters/cp-dup.tex <==
\chapter{Combinatorial Processes}




Consider the following finite population
\[
\{z_i=z_{N,i}\in\cZ, i\in[N]\}, 
\]
which is assumed non-random. The finite population distribution is then denoted by $\P_N$ and can be understood as
\[
\P_N=\frac{1}{N}\sum_{i=1}^N\delta_{z_i},~~\text{ where } \delta_z \text{ denoting the Dirac measure at } z.
\]
Suppose the sampling paradigm is uniform without replacement, yielding the following random measure that we shall call the {\it permutation measure}:
\[
\PP_{\pi,n} = \frac{1}{n}\sum_{\pi(i)\leq n}\delta_{z_i}=\frac{1}{n}\sum_{i=1}^N\delta_{z_i}\ind(\pi(i)\leq n),
\]
where $\pi$ is uniform permutation over $[N]$.

Let $\cF=\{f:\cZ\to\reals\}$ be a class of functions. This chapter is focused on the following combinatorial process that is a natural counterpart of the empirical process:
\[
\Big\{\PP_{\pi_n}f=\frac{1}{n}\sum_{i=1}^Nf(z_i)\ind(\pi\leq n); f\in\cF\Big\}.
\]
Each element in the above process has expectation
\[
\P_Nf=\frac{1}{N}\sum_{i=1}^Nf(z_i).
\]
We define
\[
\bnorm{\PP_{\pi,n}-\P_N}_{\cF}:=\sup_{f\in\cF}\Big|(\PP_{\pi,n}-\P_N)f\Big|.
\]

It is apparent that, in finite population, every random variable considered is trivially measurable so that we can drop the countability condition for $\cF$.


\section{Maximal inequalities}

\begin{lemma}\label{lem:chaining-a-and-d}
The combinatorial mean 
\[
\PP_{\pi,n}f = \sum_{i=1}^Na_{i,\pi(i)}^f=\sum_{i=1}^N\frac{f(z_i)}{n}\ind(\pi(i)\leq n)
\]
and
\[
(\PP_{\pi,n}-\P_N)f=\sum_{i=1}^N d_{i,j}^{f}=\sum_{i=1}^N\frac{f(z_i)-\P_N f}{n}\cdot \Big\{\ind(\pi(i)\leq n)-n/N\Big\}.
\]
\end{lemma}
\begin{proof}
Some straightforward algebra.
\end{proof}

\begin{lemma}[Orlicz-$\psi_2$ bounds]\label{lem:comb-orlicz} It holds true that, for any $f\in\cF$,
\[
\bnorm{(\PP_{\pi,n}-\P_N)f}_{\psi_2}\leq \sqrt{\frac{12}{n}\Big(1+\frac{N}{n}\Big)}\norm{f-\P_N f}_{L^2(\P_N)},
\]
and for any $f,g\in\cF$, 
\[
\bnorm{(\PP_{\pi,n}-\P_N)(f-g)}_{\psi_2}\leq \sqrt{\frac{48}{n}\Big(1+\frac{N}{n}\Big)}\norm{f-g}_{L^2(\P_N)}.
\]
\end{lemma}
\begin{proof}
Using Lemma \ref{lem:chaining-a-and-d}, for any $f,g\in\cF$, we have
\[
d_{i,j}^f-d_{i,j}^g=\frac{1}{n}\Big(\ind(j\leq n)-\frac{n}{N}\Big)\Big[f(z_i)-g(z_i)-\P_N(f-g)\Big].
\]
Now we will invoke Corollary \ref{cor:c-hoeffding-2}. Notice that
\begin{align}\label{eq:m-est-1}
&\frac{1}{n^2}\sup_{s\in\cS_N}\sum_{i=1}^N\Big(f(z_i)-g(z_i)-\P_N(f-g)\Big)^2\Big(\ind(s(i)\leq n)-\frac{n}{N}\Big)^2\notag\\
\leq&\frac{1}{n}\cdot\frac{N}{n}\cdot \frac{1}{N}\sum_{i=1}^N\Big(f(z_i)-g(z_i)-\P_N(f-g)\Big)^2\notag\\
\leq& \frac{1}{n}\cdot\frac{4N}{n}\P_N(f-g)^2,
\end{align}
where in the last inequality we use the Jensen's inequality to derive
\[
(\P_N (f- g))^2\leq \P_N(f-g)^2.
\]
On the other hand,
\begin{align}\label{eq:m-est-2}
&\frac{1}{N-1}\sum_{i,j\in[N]}\Big|d_{i,j}^{f}-d_{i,j}^{g}\Big|^2 \notag\\
\leq~& \frac{2}{n^2(N-1)}\sum_{i,j\in[N]}\Big(\ind(j\leq n)-\frac{n}{N}\Big)^2[f(z_i)-g(z_i)]^2\notag\\
&~~~+\frac{2}{n^2(N-1)}\sum_{i,j\in[N]}\Big(\ind(j\leq n)-\frac{n}{N}\Big)^2[\P_N(f-g)]^2\notag\\
\leq~& \frac{1}{n}\Big\{\frac{2}{N}\sum_{i=1}^N[f(z_i)-g(z_i)]^2+2[\P_N(f-g)]^2\Big\}\notag\\
\leq~& \frac{4}{n}\cdot \P_N(f-g)^2,
\end{align}
where in the last inequality we use the fact that
\[
\sum_{j=1}^N\Big(\ind(j\leq n)-\frac{n}{N}\Big)^2=\sum_{j=1}^n\Big(1-\frac{n}{N}\Big)^2+\sum_{j=n+1}^N\Big(\frac{n}{N}\Big)^2=\frac{n(N-n)}{N}.
\]
Plugging \eqref{eq:m-est-1} and \eqref{eq:m-est-2} into Corollary \ref{cor:c-hoeffding-2} and applying Lemma \ref{lem:subgaussian} yields the second claim. The first claim is similar, and is left for the readers to verify.
\end{proof}



\section{Combinatorial Glivenko-Cantelli}

\begin{definition}[$(\P_N,\pi)$-Glivenko-Cantelli] A collection of functions $\{f, f\in\cF\}$ is said to be $(\P_N,\pi)$-Glivenko-Cantelli if
\[
\E\sup_{f\in\cF}\Big|(\PP_{\pi,n}-\P_N)f\Big| \to 0.
\]
\end{definition}

\begin{theorem}[$(\P_N,\pi)$-Glivenko-Cantelli] Assume $\cF$ admits an envelope function $F>0$ such that $\limsup_{N\to\infty}\P_N F<\infty$. Suppose further that for any $\epsilon>0$, we have
\[
\lim_{N\to\infty}\frac{\log\cN(\cF,L^1(\P_N),\epsilon\norm{F}_{L^1(\P_N)})}{n}=0.
\]
It then holds true that $\cF$ is $(\P_N,\pi)$-Glivenko-Cantelli.
\end{theorem}
\begin{proof}
{\bf Step 1.} Similar to the proof of Theorem \ref{thm:gc}, for any constant $M>0$, let's introduce
\[
\cF_M:=\Big\{f\ind(F\leq M);f\in\cF\Big\}.
\]
It then holds true that
\begin{align*}
&\E\bnorm{\PP_n-\P}_{\cF} \\
\leq& \E\sup_{f\in\cF}\Big|\frac{1}{n}\sum_{\pi(i)\leq n} f(X_i)\ind(F(X_i)\leq M)-\P_Nf\ind(F\leq M)\Big|+\\
&\quad \E\sup_{f\in\cF}\Big|\frac{1}{n}\sum_{\pi(i)\leq n} f(X_i)\ind(F(X_i)> M)-\P_Nf\ind(F>M)\Big|\\
\leq& \E\bnorm{\PP_{\pi,n}-\P_N}_{\cF_M}+2\P_N F\ind(F>M).
\end{align*}


{\bf Step 2.} Now, for any $g_1,g_2\in\cF_M$ such that $\norm{g_1-g_2}_{L^1(\PP_{\pi,n})}=\PP_{\pi,n}|g_1-g_2|\leq \epsilon$, we have
\[
\Big|\frac{1}{n}\sum_{\pi(i)\leq n}g_1(X_i)-\frac{1}{n}\sum_{\pi(i)\leq n}g_2(X_i) \Big| \leq \frac{1}{n}\sum_{\pi(i)\leq n}\Big|g_1(X_i)-g_2(X_i) \Big|\leq \epsilon.
\]
Similarly, for any $g_1,g_2\in\cF_M$ such that $\norm{g_1-g_2}_{L^1(\PP_{N})}=\PP_{N}|g_1-g_2|\leq \epsilon$, we have
\[
\Big|\P_Ng_1-\P_Ng_2 \Big| \leq \P_N|g_1-g_2|\leq \epsilon.
\]

Thusly, letting $B_1,\ldots,B_{\cN(\cF_M,L^1(\PP_{\pi,n}),\epsilon)}$ denote all balls in an $\epsilon$-net of $(\cF_M,L^1(\PP_{\pi,n}))$ and $T_{\epsilon}$ denote the union of centers in the $\epsilon$-nets of $(B_j,L^1(\PP_N))$ for $j=1,\ldots,\cN(\cF_M,L^1(\PP_{\pi,n}),\epsilon)$, we then obtain
\[
\Big|T_{\epsilon} \Big| \leq \cN(\cF_M,L^1(\PP_{\pi,n}),\epsilon) \times \cN(\cF_M,L^1(\PP_N),\epsilon)
\]
and
\begin{align*}
\E\bnorm{\PP_n-\P}_{\cF} \leq \E\sup_{g\in T_{\epsilon}}\Big|(\PP_{\pi,n}-\P_N)g \Big|+2\epsilon + 2\P_N F\ind(F>M).
\end{align*}

{\bf Step 3.} Integrating Lemma \ref{lem:comb-orlicz} into Lemma \ref{lem:orlicz}, we have
\begin{align*}
&\E\sup_{g\in T_{\epsilon}}\Big|(\PP_{\pi,n}-\P_N)g \Big| \\
\leq& 2M\cdot \sqrt{\frac{12}{n}\Big(1+\frac{N}{n}\Big)}\E\sqrt{\log 2\cN(\cF_M,L^1(\PP_{\pi,n}),\epsilon)+\log 2\cN(\cF_M,L^1(\PP_N),\epsilon)}.
\end{align*}
Employing the same arguments as in the proof of Theorem \ref{thm:gc} then completes the proof.
\end{proof}



\newpage{}



\begin{corollary}\label{cor:chaining-GC1} Assume $n/N\geq r^{-1}$ for some constant $r>0$. We then have, for any $\delta>0$,
\begin{align}\label{eq:chaining-GC1-1}
\E\sup_{d_{\cF}(f,g)\leq \delta}\Big|(\PP_{\pi,n}-\P_N)(f-g)\Big|\leq \frac{16\sqrt{2}+2}{\sqrt{n}}\int_0^\delta \sqrt{\log 2\cN(\cF, d_{\cF},\epsilon)}\d \epsilon
\end{align}
and
\[
\E\sup_{f\in\cF}\Big|(\PP_{\pi,n}-\P_N)f \Big| \leq \frac{1}{\sqrt{n}}\inf_{g\in\cF}\sigma(g)+4\sqrt{\frac{2}{n}}\int_0^{\infty}\sqrt{\log 2\cN(\cF,d_{\cF},\epsilon)}\d \epsilon,
\]
where
\[
d_{\cF}^2(f,g)= 8(r+1)\P_N(f-g)^2.
\]
\end{corollary}
\begin{remark}
The assumption that $n\geq r^{-1}N$ can be dropped if a strong uniformnity condition 
\[
\frac{1}{n}\sup_{S\subset [N], |S|\leq n}\sum_{i\in S}\Big\{f(z_i)-g(z_i)-\P_N(f-g)\Big\}^2 \leq C\P_N(f-g)^2
\]
is satisfied. This condition would be easily verified in IID sampling, but no so obvious in a design setting.
\end{remark}


\begin{corollary}\label{cor:pi-GC1}
Assume 
\begin{enumerate}[label=(\roman*)]
\item $n/N\geq r^{-1}$ for some universal constant $r>0$; 
\item\label{cor:pi-GC1-2} $\inf_{g\in\cF}\sigma^2(g)=o(N)$;
\item\label{cor:pi-GC1-3} $(\cF,L_2(\P_N))$ has a bounded diameter uniformly in $N$; 
\item $\log \cN(\cF,L_2(\P_N),\epsilon)=o(N)$ as $N\to\infty$.
\end{enumerate}
The class $\cF$ is then $(\P_N,\pi)$-Glivenko-Cantelli.
\end{corollary}

\begin{example} Consider the indicator function class
\[
\cF^{\rm K}=\Big\{f_t(z)=\ind(z\leq t); t\in\mathbb{R}\Big\}.
\]
It is bounded so that Assumptions \ref{cor:pi-GC1-2} and \ref{cor:pi-GC1-3} in Corollary \ref{cor:pi-GC1} are satisfied. In addition, there can be at most $N+1$ different outputs in $\cF^{\rm K}$, so that 
\[
\log \cN(\cF,\epsilon,L_2(\P_N))=O(\log N)=o(N).
\]
Therefore, once the sampling ratio  $n/N\geq r^{-1}$, $\cF^{\rm K}$ is $(\P_N,\pi)$-Glivenko-Cantelli, which holds for {\it arbitrary} $\P_N$.
\end{example}

\section{Combinatorial Donsker}

\begin{definition}[$(\P_N,\pi)$-Donsker] Introduce 
\[
\GG^{\pi_N}f=\sqrt{n}(\PP_{\pi,n}-\P_Nf).
\] 
A collection of functions $\{f, f\in\cF\}$ is said to be $(\P_N,\pi)$-Donsker if
\[
\Big\{\GG^{\pi_N}f, f\in\cF\Big\} \Rightarrow \mathbb{G},
\]
where $\mathbb{G}$ is a tight Borel probability measure in $L^{\infty}(\cF)$.
\end{definition}



\begin{lemma}\label{lem:combinatorial-basic-Donsker} For any $f,g\in\cF$, we have
\[
\E\Big[\GG^{\pi_N}f\Big]=0, ~~~\var\Big[\GG^{\pi_N}f\Big]=\frac{N-n}{N-1}\P_N(f-\P_Nf)^2,
\]
and
\[
\cov\Big[\GG^{\pi_N}f,\GG^{\pi_N}g\Big]=\frac{N-n}{N-1}(\P_N(fg)-(\P_nf)(\P_Ng)).
\]
\end{lemma}

\begin{theorem}\label{thm:combinatorial-Donsker} Assume 
\begin{enumerate}[label=(\roman*)]
\item $\lim_{N\to\infty} n/N=\gamma\in (0,1)$;
\item there exists a probability measure $\P$ of support over the closed cover of $\cZ$ such that for any $f,g\in\cF$, 
\begin{align*}
\sup_{f\in\cF}\P|f-\P f|^3<\infty,~~~~\P_N|f-\P_Nf|^k \to \P|f-\P f|^k \text{ for }k=2,3,\\
{\rm and}~~~\P_N(fg)-\P_N(f)\P_N(g)\to \P (fg) - \P (f)\P (g);
\end{align*}
\item it holds true that
\[
\limsup_{N\to\infty}\int_0^{\infty}\sqrt{\log 2\cN(\cF,L_2(\P_N),\epsilon)}\d \epsilon<\infty.
\]
\end{enumerate}
The class $\cF$ is then $(\P_N,\pi)$-Donsker.
\end{theorem}
\begin{proof}
We use Theorem \ref{thm:EP-donsker} and Corollary \ref{cor:chaining-GC1} to prove Theorem \ref{thm:combinatorial-Donsker}. To this end, we first prove that for any finitely many functions $f_1,\ldots,f_m\in\cF$, denoting
\[
\bm{f}=(f_1,f_2,\ldots,f_m)^\top,
\]
we have
\begin{align}\label{eq:combinatorial-Donsker-1}
           \GG^{\pi_N}\bm{f} \Rightarrow N\begin{pmatrix}
         \bm{0}_m, 
         \Sigma_m
         \end{pmatrix},
\end{align}
where
\begin{align*}
[\Sigma_m]_{jk}=(1-\gamma)\cdot\P(f_j-\P f_j)(f_k-\P f_k),~~  \text{ for any }j,k\in[m].
\end{align*}
Using Lemma \ref{lem:combinatorial-basic-Donsker} and the theorem conditions, we have
\begin{align*}
&\E\GG^{\pi_N}f_k=0,\\ 
&\cov\Big[\GG^{\pi_N}f_j,\GG^{\pi_N}f_k\Big]\to (1-\gamma)\P(f_j-\P f_j)(f_k-\P f_k).
\end{align*}
Without loss of generality, we only consider those $f_j$'s such that 
\[
\P(f_j-\P f_j)^2>0.
\]

Invoking Proposition \ref{prop:mc-CLT}, to prove \eqref{eq:combinatorial-Donsker-1}, it then remains to verify the condition \eqref{eq:mc-CLT-1}, for which it is equivalent to considering
\begin{align*}
&\frac{1}{(N-1)n^{3/2}}\sum_{i,j\in[N]}\Big(\ind(j\leq n)-\frac{n}{N}\Big)^{3/2}\|\cdot \|\Sigma_m\|^{-3/2}\cdot\|\bm{f}-\P_N\bm{f}\|^{3}\\
\leq& \frac{O(1)}{n^{3/2}}\sum_{i=1}^N\Big(\sum_{j=1}^m|f_j-\P_Nf_j|^2\Big)^{3/2}\\
=& O(N^{-1/2}),
\end{align*}
where in the last equality we used the fact that 
\[ 
\P_N|f_j-\P_N f_j|^3 \to \P|f_j-\P f_j|^3<\infty~~\text{ for any }j\in[m].
\] 
This verifies \eqref{eq:combinatorial-Donsker-1}. 

On the other hand, stochastic equicontinuity  can be directly verified by invoking Corollary \ref{cor:chaining-GC1}, using Condition \eqref{eq:chaining-GC1-1}, and employing dominated convergence theorem.
\end{proof}


\begin{corollary}[Uniform entropy argument] Assume the first two conditions in Theorem \ref{thm:combinatorial-Donsker} hold. If in addition $\cF$ admits an envelope function $F>0$ such that
\[
|f(z)| \leq F(z)~~~\text{ for all }f\in\cF \text{ and }z\in\cZ
\]
and 
\[
\limsup_{N\to\infty}\P_N F^2<\infty.
\] 
We then have, if $\cF$ further satisfies 
\[
\int_0^{1}\sup_Q\sqrt{\log 2\cN(\cF,L_2(Q),\epsilon\|F\|_{L_2(Q)})}\d \epsilon<\infty,
\]
where the supremum is taken over all finitely discrete probability measure, then $\cF$ is $(\P_N,\pi)$-Donsker.
\end{corollary}
\begin{proof}
We have
\begin{align*}
&\limsup_{N\to\infty}\int_0^{\infty}\sqrt{\log 2\cN(\cF,L_2(\P_N),\epsilon)}\d \epsilon \\
=&\limsup_{N\to\infty}\int_0^{\norm{F}_{L_2(\P_N)}}\sqrt{\log 2\cN(\cF,L_2(\P_N),\epsilon)}\d \epsilon \\
=& \limsup_{N\to\infty}\norm{F}_{L_2(\P_N)}\int_0^{1}\sqrt{\log 2\cN(\cF,L_2(\P_N),\epsilon\norm{F}_{L_2(\P_N)})}\d \epsilon\\
\leq& \limsup_{N\to\infty} \norm{F}_{L_2(\P_N)}\cdot \int_0^{1}\sup_Q\sqrt{\log 2\cN(\cF,L_2(Q),\epsilon\|F\|_{L_2(Q)})}\d \epsilon\\
<&\infty,
\end{align*}
which completes the proof.
\end{proof}


\section{Bernstein chaining}

The requirement that $n/N>r^{-1}$ in Corollary \ref{cor:chaining-GC1} and many subsequent parts are unnecessary. The reason for adding this condition is the use of a loose combinatorial moment bound, Corollary \ref{cor:c-hoeffding-2}, throughout the above sections. 

For strengthening the above bounds, on the other hand, some additional efforts are needed. To this end, for any nondecreasing convex function $\psi$ such that $\psi(0)=0 $, let's introduce the corresponding Orlicz norm $\norm{\cdot}_{\psi}$ to be
\[
\norm{X}_{\psi} =\inf\Big\{C>0: \E\psi\Big(\frac{|X|}{C}\Big)\leq 1 \Big\}.
\]
Two particularly useful choices of the $\psi$ is 
\[
\psi_1(x)=e^{x}-1~~~{\rm and}~~~\psi_2(x)=e^{x^2}-1,
\]
corresponding to the subgaussian and subexponential random variables.

The following is the famous Dudley chaining bound.
\begin{theorem}\label{thm:dudley}
Consider $\{X(t);t\in\cT\}$ to be a separable process and $(\cT,d)$ to be a pseudo-metric space such that
\[
\norm{X(t)-X(s)}_{\psi_p}\leq d(s,t),~~~\text{ for all }s,t\in\cT,
\]
where $p\in [2]$. Then, 
\[
\E\sup_{s,t\in\cT}|X(t)-X(s)| \leq 8\int_0^{\infty}\psi_p^{-1}\Big(\cN(\cT,d,\epsilon)\Big)\d \epsilon 
\]
where $K$ only depends on $C$ and $p$.
\end{theorem}
\begin{proof}
Section A.5 in \cite{talagrand2014upper} and Theorem 11.1 in \cite{ledoux2013probability}.
\end{proof}

It is easy to see that, when choosing $p=2$, Theorem \ref{thm:dudley} reduces to Theorem \ref{thm:chaining}. The prime interest of this section, on the other hand, is when $p=1$, which corresponds to the subexponential case. 

The following lemma will be of interest to us.
\begin{lemma}\label{lem:berstein-orlicz}
Suppose $X_1,\ldots,X_m$ have Bernstein-type bounds such that that
\[
\P(|X_k|>t)\leq 2\exp\Big(-\frac{t^2}{2(B^2+At)}\Big), ~~\text{ for all }t>0 \text{ and }k\in[m].
\]
There then exists a universal constant $C>0$ such that
\[
\norm{X}_{\psi_1}\leq C(A\log 2m+B\sqrt{\log 2m}).
\]
\end{lemma}
\begin{proof}
Lemma 2.2.10 of \cite{vaart2023empirical}.
\end{proof}

Combining the above lemma with Theorem \ref{thm:cb-ineq} then yields the following bound.
\begin{proposition} For any $f,g\in\cF$, it holds true that
\[
\norm{\GG^{\pi_N}(f-g)}_{\psi_1}\leq K\Big(\norm{f-g}_{L_2(\P_N)}+\frac{1}{\sqrt{n}}\norm{f-g}_{\infty}\Big).
\]
\end{proposition}
\begin{proof}
Plugging Lemma \ref{lem:chaining-a-and-d} into Theorem \ref{thm:cb-ineq} and combining it with Lemma \ref{lem:berstein-orlicz} yields the conclusion.
\end{proof}

\begin{corollary} There exists a universal constant $C>0$ such that, for any $\delta>0$,
\[
\E\sup_{d(f,g)<\delta}|\GG^{\pi_N}(f-g)|\leq C\int_0^{\delta}\log2\cN(\cF,d,\epsilon)\d \epsilon,
\]
where
\[
d(f,g)=\norm{f-g}_{L_2(\P_N)}+\frac{1}{\sqrt{n}}\norm{f-g}_{\infty}.
\]
\end{corollary}


\begin{corollary}
Assume only the second condition in Theorem \ref{thm:combinatorial-Donsker} holds. If in addition $\cF$ admits an envelope function $F>0$ such that
\[
|f(z)| \leq F(z)~~~\text{ for all }f\in\cF \text{ and }z\in\cZ
\]
and 
\[
\limsup_{N\to\infty}\P_N F^2<\infty.
\] 
We then have, if $\cF$ further satisfies 
\[
\int_0^{1}\log 2\cN(\cF,L_{\infty},\epsilon\|F\|_{\infty})\d \epsilon<\infty,
\]
then $\cF$ is $(\P_N,\pi)$-Donsker.
\end{corollary}


\section{Bracketing chaining}

\begin{lemma}
Let $f_1,\ldots,f_m \in\cF$ such that 
\[
\max_{k\in[m]}\norm{f_k-\P_N f_k}_{\infty}\leq c<\infty
\] 
and denote $\sigma^2:=\max_{k\in[r]}\P_N(f_k-\P_Nf_k)^2$. There then exists a universal constant $K>0$ such that
\[
\norm{\max_{k\in[m]} |f_k-\P_Nf_k|}_{\psi_1} \leq K\Big(\sqrt{\frac{\sigma^2\log (2m)}{n}}+cn\log (2n) \Big).
\]
\end{lemma}
\begin{proof}
Combining Theorem \ref{thm:cb-ineq} and Lemma \ref{lem:berstein-orlicz} yields the conclusion.
\end{proof}

\begin{corollary}[Bracketing entropy bounds] Assume $\cF$ admits an envelope function $F$ such that 
\[
\norm{F}_{\infty}<\infty ~~\text{ and } \sup_{f\in\cF}\P_Nf^2<\delta<\infty
\]
for some constant $\delta>0$. There then exists a universal constant $K>0$ such that
\[
\E\sup_{f\in\cF}|\GG^{\pi_N}f| \leq K\Big( 1+\frac{\norm{F}_{\infty}}{\sqrt{n}\delta^2}\int_0^{2\delta}\sqrt{\log 2\cN_{[]}(\cF,L_2(\PP_N),\epsilon)}\d \epsilon\Big)\cdot \int_0^{2\delta}\sqrt{\log 2\cN_{[]}(\cF,L_2(\PP_N),\epsilon)}\d \epsilon
\]
\end{corollary}
\begin{proof}
Proposition 3.5.15 in \cite{gine2021mathematical}.
\end{proof}


\section{Generic chaining bounds}

Define
\[
N_0=1, N_n=2^{2^n} \text{ for }n\geq 1,
\]

\begin{definition}
For any pseudo-metric space $(\cT,d)$, any $t\in\cT$, and any $T_n\subset\cT$, let 's define 
\[
d(t,T_n)=\inf_{s\in T_n}d(t,s)~~~{\rm and}~~~e_n(\cT,d)=\inf_{T_n}\sup_{t}d(t,T_n),
\]
where the infimum is taken over all $|T_n|\leq N_n$.
\end{definition}


\begin{definition}
For any pseudo-metric space $(\cT,d)$ and any $\alpha>0$, define
\[
\gamma_{\alpha}(\cT,d)=\inf\sup_{t\in\cT}\sum_{n\geq 0}2^{n/\alpha}\diam(A_n(t)),
\]
where the infimum is taken over all increasing sequences $\cA_n$ of partitions of $\cT$ such that $|\cA_n|\leq N_n$, and $A_n(t)$ denotes the unique element in $\cA_n$ that contains $t$. 
\end{definition}

\begin{theorem}[Bernstein chaining] Consider $\cT$ to be equipped with two metrics $d_1,d_2$ such that the process $\{X(t);t\in\cT\}$ satisfies
\begin{align}\label{eq:bchaining-condition}
\P(|X(s)-X(t)|\geq u)\leq 2\exp\Big(-\frac{u^2/2}{d_2(s,t)^2+ud_1(s,t)}  \Big),~~\text{for all }s,t\in\cT \text{ and }u>0.
\end{align}
There then exists a universal constant $K>0$ such that
\[
\E\sup_{s,t\in\cT}|X(s)-X(t)|\leq K(\gamma_1(\cT,d_1)+\gamma_2(\cT,d_2)).
\]
\end{theorem}
\begin{proof}
Theorem 2.2.23 in \cite{talagrand2014upper}.
\end{proof}

\begin{corollary} Consider the stochastic process $\{X(t);t\in\cT\}$ that satisfies Condition \eqref{eq:bchaining-condition}. It then holds true that
\[
\E\sup_{s,t\in\cT}|X(s)-X(t)|\leq K\Big(\int_0^{\infty}\sqrt{\log 2\cN(\cT,d_2,\epsilon)}\d \epsilon + \int_0^{\infty}\log 2\cN(\cT,d_1,\epsilon)\d \epsilon\Big),
\]
where $K>0$ is a universal constant.
\end{corollary}
\begin{proof}
The proof is based on the following lemma that connects $\gamma_{\alpha}(\cT,d)$ to $e_n(\cT,d)$.
\begin{lemma} For any $\alpha>0$ and any metric space $(\cT,d)$, it holds true that
\[
\gamma_{\alpha}(\cT,d)\leq K(\alpha)\sum_{n\geq 0}2^{n/\alpha}e_n(\cT,d).
\]
\end{lemma}
Using the above lemma, we could then separately bound $\gamma_1(\cT,d_1)$ and $\gamma_2(\cT,d_2)$. 

{\bf Bounding $\gamma_2(\cT,d_2)$.} Noticing that 
\[
e_n(\cT,d_2)=\inf\Big\{\epsilon: \cN(\cT,d_2,\epsilon)\leq N_n  \Big\},
\]
we obtain
\[
\epsilon<e_n(\cT,d_2) \text{ implies }\cN(\cT,d_2,\epsilon)\geq 1+N_n.
\]
Accordingly, we have
\begin{align*}
\int_{e_{n+1}(\cT,d_2)}^{e_n(\cT,d_2)}\sqrt{\log\cN(\cT,d_2,\epsilon)}\d\epsilon &\geq \sqrt{\log(1+N_n)}(e_n(\cT,d_2)-e_{n+1}(\cT,d_2))\\
&\geq \sqrt{\log 2}\cdot 2^{n/2}(e_n(\cT,d_2)-e_{n+1}(\cT,d_2)),
\end{align*}
where in the second inequality we use the fact that 
\[
\log(1+N_n)\geq 2^n\log 2.
\]
Summing over all $n\geq 0$, we obtain
\begin{align*}
\int_0^{e_0(\cT,d_2)}\sqrt{\log \cN(\cT,d_2,\epsilon)}\d\epsilon\geq& \sqrt{\log 2}\sum_{n\geq 0}2^{n/2}(e_n(\cT,d_2)-e_{n+1}(\cT,d_2))\\
\geq & \Big(1-\frac{1}{\sqrt{2}}\Big)\sqrt{\log 2}\sum_{n\geq 0}2^{n/2}e_n(\cT,d_2),
\end{align*}
which gives the desired bound that
\[
\gamma_2(\cT,d_2)\leq K\int_0^{\infty}\sqrt{\log 2\cN(\cT,d_2,\epsilon)}\d\epsilon.
\]

{\bf Bounding $\gamma_1(\cT,d_1)$.} The derivation is similar. We have
\begin{align*}
\int_{e_{n+1}(\cT,d_1)}^{e_n(\cT,d_1)}\log\cN(\cT,d_1,\epsilon)\d\epsilon &\geq \log(1+N_n)(e_n(\cT,d_1)-e_{n+1}(\cT,d_1))\\
&\geq \log 2\cdot 2^{n}(e_n(\cT,d_1)-e_{n+1}(\cT,d_1)),
\end{align*}
implying
\begin{align*}
\int_0^{e_0(\cT,d_1)}\log \cN(\cT,d_1,\epsilon)\d\epsilon\geq& \log 2\sum_{n\geq 0}2^{n}(e_n(\cT,d_1)-e_{n+1}(\cT,d_1))\\
= & \frac{\log 2}{2}\sum_{n\geq 0}2^{n}e_n(\cT,d_1),
\end{align*}
so that
\[
\gamma_1(\cT,d_1)\leq K\int_0^{\infty}\log 2\cN(\cT,d_1,\epsilon)\d\epsilon.
\]
\end{proof}

\begin{corollary} There exists a universal constant $C>0$ such that, for any $\delta>0$,
\[
\E\sup_{d(f,g)<\delta}|\GG^{\pi_N}(f-g)|\lesssim \int_0^{\delta}\sqrt{\log2\cN(\cF,L^2(\P_N),\epsilon)}\d \epsilon+\frac{1}{n}\int_0^{\delta}\log 2\cN(\cF,L^{\infty}(\P_N),\epsilon)\d \epsilon.
\]



\end{corollary}



==> chapters/nonp-reg.tex <==
\chapter{Finite-population nonparametric regression}
\label{chapter:nonp-reg}

In classic nonparametric regression, we have access to $n$ IID observations, $(Y_1,\bX_1),\ldots, (Y_n,\bX_n)$ of a pair $(Y,\bX)\in \reals \times \reals^d$, and the goal of interest is to estimate
\[
\psi(\bx)=\E[Y\mid \bX=\bx]
\]
based on the observations $\{(Y_i,\bX_i), i\in[n]\}$.

In a finite-population nonparametric regression case, we assume there exists a finite population
\[
(y_1,\bx_1),\ldots,(y_N,\bx_N),
\]
while what we observed is a randomly sampled size-$n$ subset of it. Using the permutation notation, the sample is
\[
\Big\{(y_i,\bx_i), \pi(i)\leq n\Big\}.
\]

Since the population size is finite, the conditional expectation $\E_{\P_N}(Y \mid \bX=\bx)$ is rarely of any statistical meaning. Instead, let's directly compare the nonparametric regression estimate over $\P^{\pi_N}$ compared to that over the population $\P_N$.


In detail, consider 
\[
\bp_K(\bx)=(p_{1K}(\bx),\ldots,p_{KK}(\bx))^\top
\]
to be a $K$-dimensional vector of basis functions 
\[
p_{jk}(\cdot): \reals^d\to\reals.
\]
The series estimator based on the random sample $\{(y_i,\bx_i), \pi(i)\leq n\}$ is
\[
\hat\psi_K(\bx)=\bp_K(\bx)^\top\hat\bbeta_K,~~~\hat\bbeta_K\in \argmin\limits_{\bb\in\reals^K}\frac{1}{n}\sum_{i=1}^N(Y_i-\bp_K(\bx_i)^\top\bb)^2\ind(\pi(i)\leq n),
\]
which should approximate its population counterpart
\[
\psi_K(\bx)=\bp_K^\top(\bx)\bbeta_K,~~~\bbeta_K\in \argmin\limits_{\bb\in\reals^K}\frac{1}{N}\sum_{i=1}^N(Y_i-\bp_K^\top(\bx_i)\bb)^2.
\]

Let $\Ab^-$ be the generalized inverse of the matrix $\Ab$. It is clear that 
\begin{align*}
\hat\bbeta_K = (\Pb_{\pi}^\top\Pb_{\pi})^{-}\Pb_{\pi}^\top\bY,~~~{\rm with}~\bY=(y_1,\ldots,y_N)^\top,\\
{\rm and}~~~\Pb_{\pi}=(\bp_K(\bx_1)\ind(\pi(1)\leq n),\ldots,\bp_K(\bx_N)\ind(\pi(N)\leq n))^\top.
\end{align*}
Additionally, denoting 
\[
\Pb_N=(\bp_K(\bx_1),\ldots,\bp_K(\bx_N))^\top~~~{\rm and}~~~\Qb=\Pb_N^\top\Pb_N/N=\P_N[\bp_K(\bx)\bp_K^\top(\bx)],
\]
we have
\[
\bbeta_K=\Qb^{-}\cdot\frac{\Pb_N^\top\bY}{N}.
\]
Let $\zeta_{q,K}=\max_{\bt\in\Lambda_q}\sup_{\bx\in \cX}\norm{\partial^{\bt}\bp_K(\bx)}$.

\begin{theorem}\label{thm:nonp-reg} Assume $\pi$ is a uniform random permutation, $\lambda_K=\lambda_{\min}(\Qb)>0$, and
\[
(1+\lambda_K^{-1}\zeta_{0,K})^2\log K/n\to 0.
\]
We have
\[
\P_N(\hat\psi_K-\psi_K)^2=O_{\P^{\pi_N}}\Big(\lambda_K^{-1}(A_N^2\gamma_N+B_N^2) \Big),
\]
where
\begin{align*}
A_N=(1+\lambda_K^{-1/2}\zeta_{0,k})\sqrt{\frac{\log K}{n}}+(1+\lambda_K^{-1}\zeta_{0,K}^2)\frac{\log K}{n}, ~~\gamma_N=\norm{\P_N[y\bp_K(\bx)]}^2,
\end{align*}
and
\[
B_N^2= \frac{2}{n}\sum_{j=1}^K\P_N\Big(y_ip_{kj}-\P_N\Big[yp_{Kj}(\bx)\Big]\Big)^2.
\]
\end{theorem}
\begin{proof}

Introduce $\hat\Qb=\Pb_{\pi}^\top\Pb_{\pi}/n$. We have the following lemma.
\begin{lemma}\label{lem:nonp-reg-lem1} It holds true that
\[
\E\bnorm{\Qb^{-1/2}\hat\Qb\Qb^{-1/2}-\Ib_K}_\op \lesssim A_N.
\]
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:nonp-reg-lem1}]
Notice that
\[
\hat\Qb=\frac{1}{n}\sum_{i=1}^N\bp_K(\bx_i)\bp_K(\bx_i)^\top\ind(\pi(i)\leq n).
\]
It is immediate that
\begin{align*}
\Qb^{-1/2}\hat\Qb\Qb^{-1/2}-\Ib_K&=\frac{1}{n}\sum_{i=1}^N\Qb^{-1/2}\bp_K(\bx_i)\bp_K^\top(\bx_i)\Qb^{-1/2}\ind(\pi(i)\leq n)-\Ib_K\\
&=\sum_{i=1}^n \Ab_{i,\pi(i)}
\end{align*}
with
\[
\Ab_{i,j}=\frac{1}{n}\Big(\Qb^{-1/2}\bp_K(\bx_i)\bp_K^\top(\bx_i)\Qb^{-1/2}-\Ib_K\Big)\ind(j\leq n),
\]
whose expectation is easy to be checked to be $\bm{0}$. Additionally, we have
\[
\bnorm{\Ab_{i,j}}_\op \leq \frac{1}{n}\Big(1+\lambda_K^{-1}\zeta_{0,K}^2\Big)
\]
and
\[
\frac{1}{N}\bnorm{\sum_{i,j\in[N]}\Ab_{i,j}^2}_\op \leq \frac{1}{n}\Big(1+3\lambda_K^{-1}\zeta_{0,K}^2\Big).
\]
This is because, since $\lambda_K=\lambda_{\min}(\Qb)>0$, it holds true that 
\[
\norm{\Qb^{-1/2}}_\op=\lambda_K^{-1/2}<\infty,
\]
and thus
\[
\bnorm{\Qb^{-1/2}\bp_K(\bx_i)\bp_K(\bx_i)^\top\Qb^{-1/2}}_\op = \bnorm{\Qb^{-1/2}\bp_K(\bx_i)}^2\leq \lambda_K^{-1}\zeta_{0,K}^2,
\]
and 
\begin{align*}
&\bnorm{\P_N\Big[\Qb^{-1/2}\bp_K(\bx_i)\bp_K(\bx_i)^\top\Qb^{-1}\bp_K(\bx_i)\bp_K(\bx_i)^\top\Qb^{-1/2}  \Big]}_\op^2\\
\leq & \lambda_K^{-1}\zeta_{0,K}^2\bnorm{\P_N\Big[\Qb^{-1/2}\bp_K(\bx_i)\bp_K(\bx_i)^\top\Qb^{-1/2} \Big]}\\
= & \lambda_K^{-1}\zeta_{0,K}^2.
\end{align*}
Accordingly, invoking Theorem \ref{thm:cmbi} yields the claim.
\end{proof}

Getting back to the proof of Theorem \ref{thm:nonp-reg}, defining
\[
A_n=\Big\{\lambda_{\min}(\Qb^{-1/2}\hat\Qb\Qb^{-1/2})>1/2\Big\},
\]
we have
\begin{align*}
&\ind_{A_n}\P_N(\hat\psi_K-\psi_K)^2 \\
=& \ind_{A_n}\P_N[\bp_K^\top(\bx)\hat\bbeta_K-\bp_K^\top(\bx)\bbeta_K]^2\\
=& \ind_{A_n}(\hat\bbeta_K-\bbeta_K)^\top\Qb(\hat\bbeta_K-\bbeta_K)\\
=&\ind_{A_n}\bnorm{\Qb^{1/2}(\hat\bbeta_K-\beta_K)}^2\\
\leq& 2\ind_{A_n}\bnorm{\Qb^{1/2}\Big[\hat\Qb^{-1}-\Qb^{-1}\Big]\frac{\Pb_{\pi}^\top\bY}{n}}^2+2\ind_{A_n}\bnorm{\Qb^{-1/2}\Big[\frac{\Pb_\pi^\top\bY}{n}-\frac{\Pb_N^\top\bY}{N}}^2\\
=&2\ind_{A_n}\bnorm{\Big[\Qb^{1/2}\hat\Qb^{-1}\Qb^{1/2}-\Ib_K\Big]\Qb^{-1/2}\frac{\Pb_{\pi}^\top\bY}{n}}^2+2\ind_{A_n}\bnorm{\Qb^{-1/2}\Big[\frac{\Pb_\pi^\top\bY}{n}-\frac{\Pb_N^\top\bY}{N}}^2\\
\leq&2\ind_{A_n}\lambda_K^{-1}\Big(\bnorm{\Qb^{-1/2}\hat\Qb^{-1}\Qb^{1/2}-\Ib_K}_{\op}^2\bnorm{\frac{\Pb_{\pi}^\top\bY}{n}}^2+\bnorm{\frac{\Pb_\pi^\top\bY}{n}-\frac{\Pb_N^\top\bY}{N}}^2\Big).
\end{align*}

\begin{lemma}
If $\norm{\Ab-\Ib}_\op\leq \lambda<1$, then $\norm{\Ab^{-1}-\Ib}_{\op} \leq \frac{\lambda}{1-\lambda}$.
\end{lemma}

Using the above lemma and noticing that
\[
\ind_{A_n}\Big(\Qb^{-1/2}\hat\Qb\Qb^{-1/2}\Big)^{-1}=\ind_{A_n}\Qb^{1/2}\hat\Qb^{-1}\Qb^{1/2},
\]
we obtain that 
\[
\ind_{A_n}\norm{\Qb^{-1/2}\hat\Qb^{-1}\Qb^{1/2}-\Ib_K}_{\op}=O_{\P^{\pi_N}}\Big((1+\lambda_K^{-1/2}\zeta_{0,k})\sqrt{\frac{\log K}{n}}+(1+\lambda_K^{-1}\zeta_{0,K}^2)\frac{\log K}{n} \Big).
\]

\begin{lemma}
We have 
\[
\E\bnorm{\frac{\Pb_\pi^\top\bY}{n}-\frac{\Pb_N^\top\bY}{N}}^2 \leq \frac{2}{n}\sum_{j=1}^K\P_N\Big(y_ip_{kj}-\P_N\Big[yp_{Kj}(\bx)\Big]\Big)^2=B_N^2.
\]
\end{lemma}
\begin{proof}
We have
\begin{align*}
&\E\bnorm{\frac{\Pb_\pi^\top\bY}{n}-\frac{\Pb_N^\top\bY}{N}}^2\\
=&\E\bnorm{\frac{1}{n}\sum_{i=1}^N\Big(y_i\bp_K(\bx_i)-\P_N[y\bp_K(\bx)]\Big)\ind(\pi(i)\leq n)}^2\\
=&\sum_{j=1}^K\E\Big|\frac{1}{n}\sum_{i=1}^N\Big(y_ip_{Kj}(\bx_i)-\P_N[yp_{Kj}(\bx)]\Big)\ind(\pi(i)\leq n)  \Big|^2\\
\leq & \frac{2}{n}\sum_{j=1}^K\P_N\Big(y_ip_{kj}-\P_N\Big[yp_{Kj}(\bx)\Big]\Big)^2.
\end{align*}
\end{proof}
Using the above lemma completes the proof.
\end{proof}

==> chapters/rbs.tex <==
\chapter{Rank-based Statistics}
\label{chapter:rbs}


